Towards Automated Driving Violation Cause Analysis in Scenario-Based Testing for Autonomous Driving Systems

The rapid advancement of Autonomous Vehicles (AVs), exemplified by companies like Waymo and Cruise offering 24/7 paid taxi services, highlights the paramount importance of ensuring AVs' compliance with various policies, such as safety regulations, traffic rules, and mission directives. Despite significant progress in the development of Autonomous Driving System (ADS) testing tools, there has been a notable absence of research on attributing the causes of driving violations. Counterfactual causality analysis has emerged as a promising approach for identifying the root cause of program failures. While it has demonstrated effectiveness in pinpointing error-inducing inputs, its direct application to the AV context to determine which computation result, generated by which component, serves as the root cause poses a considerable challenge. A key obstacle lies in our inability to straightforwardly eliminate the influence of a specific internal message to establish the causal relationship between the output of each component and a system-level driving violation. In this work, we propose a novel driving violation cause analysis (DVCA) tool. We design idealized component substitutes to enable counterfactual analysis of ADS components by leveraging the unique opportunity provided by the simulation. We evaluate our tool on a benchmark with real bugs and injected faults. The results show that our tool can achieve perfect component-level attribution accuracy (100%) and almost (>98%) perfect message-level accuracy. Our tool can reduce the debugging scope from hundreds of complicated interdependent messages to one single computation result generated by one component.

==> Tables/benchmark_table.tex <==
% % \usepackage{multirow}

% \begin{wraptable}{r}{10cm}
% \centering
% \footnotesize
% \caption{Benchmark for evaluating cause localization tool. We list all the applied Collision Scenario (CS) for each type of injected fault. For each applied CS in the table, we create a corresponding collision instance.}

% \begin{tabular}{l|l|l}
% \hline
% \textbf{Component}           & \textbf{Injected error}                & \textbf{Applied CS}    \\
% \hline
% \multirow{5}{*}{Perception}                & Miss object detection result  & 1, 2, 3, 4    \\
%                           & Wrong bounding box estimation & 4             \\
%                           & Wrong longitudinal distance   & 1, 2, 3, 4    \\
%                           & Wrong lateral distance        & 1, 2, 3, 4    \\
%                           & Wrong velocity measurement    & 1, 2, 3, 4    \\
% \hline
% \multirow{2}{*}{Prediction}                & No prediction trajectory      & 1             \\
%                           & Wrong prediction trajectory   & 1, 2, 3, 4    \\
% \hline
% \multirow{3}{*}{Planning} & Incorrect path planning       & 3, 4, 5       \\
%                           & Incorrect speed planning      & 1, 2, 3       \\
%                           & No planning trajectory        & 1, 2, 3, 4, 5 \\
% \hline
% \multirow{2}{*}{Control}  & Wrong longitudinal command    & 1, 2, 3, 4    \\
%                           & Wrong lateral command         & 5             \\
% \hline
% Localization              & Wrong lateral localization    & 5           \\
% \hline

% \end{tabular}
% \label{tab:benchmark}
% \end{wraptable}

==> Tables/injected_results.tex <==
\begin{wraptable}{r}{0.7\textwidth}
\footnotesize
\begin{tabular}{lllll}
\hline
             & \begin{tabular}[c]{@{}l@{}}Component-level\\ success rate\end{tabular} & \begin{tabular}[c]{@{}l@{}}Message-level\\ success rate\end{tabular} & \begin{tabular}[c]{@{}l@{}}Average \\ reduction rate\end{tabular} & \begin{tabular}[c]{@{}l@{}}Average \\ time (min)\end{tabular} \\ \hline
Perception   & 100\%                                                                  & 100\%                                                                & 0.11\%                                                            & 17.2                                                          \\ \hline
Prediction   & 100\%                                                                  & 100\%                                                                & 0.09\%                                                            & 15.1                                                          \\ \hline
Planning     & 100\%                                                                  & 100\%                                                                & 0.13\%                                                            & 2.7                                                           \\ \hline
Control      & 100\%                                                                  & 80\%                                                                 & 21.3\%                                                            & 20.3                                                          \\ \hline
Localization & 100\%                                                                  & 100\%                                                                & 1.37\%                                                            & 19.6                                                          \\ \hline
\end{tabular}
\end{wraptable}

==> Tables/real_results.tex <==
\begin{wraptable}{r}{0.4\textwidth} % {对齐方式}{宽度}
\footnotesize
\label{tab:real_result}
\begin{tabular}{lllll}
\hline
ID & \begin{tabular}[c]{@{}l@{}}Component-\\level success\end{tabular} & \begin{tabular}[c]{@{}l@{}}Message-\\level success\end{tabular} & \begin{tabular}[c]{@{}l@{}}Reduction\\rate\end{tabular} & \begin{tabular}[c]{@{}l@{}}Time\\(min))\end{tabular} \\ \hline
1     & Y                                                                 & Y                                                               & 1.3\%          & 3.1        \\ \hline
2     & Y                                                                 & Y                                                               & 0.4\%          & 17.2       \\ \hline
3     & Y                                                                 & Y                                                               & 0.9\%          & 2.2        \\ \hline
4     & Y                                                                 & Y                                                               & 1.5\%          & 3.8        \\ \hline
5     & Y                                                                 & Y                                                               & 1.1\%          & 3.1        \\ \hline
6     & Y                                                                 & Y                                                               & 0.7\%          & 2.9        \\ \hline
7     & Y                                                                 & Y                                                               & 1.2\%          & 2.4        \\ \hline
8     & Y                                                                 & Y                                                               & 1.1\%          & 3.0        \\ \hline
\end{tabular}
\end{wraptable}

==> design_prev.tex <==
\section{System Design}
\label{sec:design}

\begin{figure*}[t]
    \centering
    \includegraphics[width=\linewidth]{overview.pdf}
    \caption{Overview of design. We use message-level as an example to demonstrate the whole framework. For component-level localization, the framework remains the same except that the counterfactual analysis is based on components instead of messages. \alfred{for the ``message record'' box on the left, not sure what different rows mean; on the ``Cause localization algorithm'' box: label state numbers, use dotted line to separate different steps.}}
    \label{fig:framework}
\end{figure*}

 


\subsection{Design Overview}
\label{design:overview}

In this section, we will present our high-level solution idea and an overview of our concrete automated SVCA tool design. 

\textbf{Key solution principle: Counterfactual causality.} To address \textbf{C1}, our key idea is built upon the principle of \textit{counterfactual causality}~\cite{lewis2013counterfactuals} to establish provable causal relationship between ADS system-level safety violation and component-level errors. In particular, it infers the causality via f counterfactual conditionals: ``If X had not occurred, Y would not have occurred''. Specifically, in our context of cause attribution in ADS, if a certain set of messages is not executed in the simulation testing, and the collision does not happen anymore, then the collision is causally dependent on the fault in that specific component.

\textbf{System inputs and outputs.} Following the idea of counterfactual causality, we start to formulate our problem inputs and outputs.  We define the simulation testing as function $test : S \rightarrow \{ \cmark, \xmark \}$, where $S$ is the set of all traffic scenarios, and~\cmark, \xmark ~ means the safety violation does not happen and happens correspondingly. The \textbf{inputs} to our system is a safety violation scenario $S_{viol}$ where \begin{equation}
    test(S_{viol}) = \xmark
\end{equation}
To enable the counterfactual analysis, we define function $rtest$ for this specific safety-violation scenario $\mathit{rtest}: M \rightarrow \{\cmark, \xmark \}$ to \rhl{determine the simulation testing result if a set of messages $M$ will not occur in the testing anymore}. \josh{I don't understand the highlighted text in the previous sentence.} 
The component-level cause attribution task is to find a local minimum set of components $\mathit{faulty}\_components$ such that \begin{equation}
    rtest(M_{\mathit{faulty}\_components}) = \cmark
\end{equation}
where $M_{\mathit{faulty}\_components}$ is the collection of all output messages of faulty components. We follow the same definition of local minimum in prior work~\cite{zeller2002simplifying}. \josh{You still need text here explaining what you mean by local minimum. This paper still needs to be self-contained.} Similarly, the message-level cause attribution task is to find a local minimum set of messages $M_{\mathit{faulty}\_messages}$ such that \begin{equation}
    rtest(M_{\mathit{faulty}\_messages}) = \cmark
\end{equation}


\textbf{Tool design overview.} Fig.~\ref{fig:framework} show an overview of our tool design. As shown, the input of the tool is a safety-violation scenario. To enable the counterfactual analysis, we need to find \textit{idealized substitutes} for each ADS component so that we can analyze the counterfactual relationship between messages and safety violations. In order to analyze the testing results excluding some component outputs in function $rtest$, we need to replace the original output messages with those from the idealized component substitutes (i.e., the ideal outputs without component-level errors).

With the provable causal relationship establishment capability, we still need to address the component-level message non-determinism across different runs of the same test case (\textbf{C2}) to enable counterfactual analysis at the message level. To address this, we propose to construct a novel \textit{mapping} algorithm between the semantically-equivalent messages across the different runs of the same test case. To systematically achieve this, our key idea is to exploit the vehicle dynamic states (more details in~\S\ref{design:state}) to map messages among different tests. \josh{I think you mean ``tests''.} The recorded messages will be clustered based on vehicle dynamic states and also our cause attribution algorithm will control the configuration of counterfactual analysis to gradually attribute the cause. In the following sections, we will detail these key novel design components.

\cut{
\textbf{Key.} We identified two unique challenges in designing an automated tool to attribute cause of faults in AD system. 
\textbf{C1. We need to find idealized substitutes for each component in AD software stack so that we can analyze the counterfactual relationship between messages and safety-violation.} In order to analyze the testing results excluding some component outputs in function $rtest$, we need to replace the original output messages with idealized substitutes (i.e., the expected outputs without fault).
\textbf{C2. Due to the randomness of testing, we can not find exactly the same messages across different simulation testing execution.} Thus, we need to construct a mapping between messages in different executions. We provides an example to illustrate the unique randomness in simulation testing in Fig.~\ref{fig:exec_diff}. We extract the time and driving distance of ego vehicle for each planning component execution under exactly the same testing scenario. We use different colors (light blue and dark blue) to for different testing cases. Even though the trajectory of two cases can align well, the time and vehicle position still vary among two executions, meaning the inputs (e.g., vehicle localization, sensor data) to the AD components will also be different. As a result, we can not directly remove one message in next testing since it may not exist in another testing case.
}



\subsection{Idealized Substitute Design for ADS Components}
\label{design:ideal_sub}
To address \textbf{C1}, we designed idealized component substitutes for each component in the ADS. Our idealized component substitute should behave as design expectation or try its best to avoid the safety violation. Our design can be classified as two types: 

\textbf{1. Extending simulation bridge interface.} We discovered that simulation testing brings new opportunities for counterfactual analysis. The common usage of simulation is that it will interact with AD software with raw sensor data and control command which will be executed by actuators. However, we discover that a lot of intermediate results can be directly extracted or executed by the simulator, which enables the design of idealized substitutes of perception, prediction, control, and localization components. 

We illustrate the design details of idealized substitutes \josh{I think you mean ``substitutes''} of 4 components in Fig.~\ref{fig:idea_sub}. The localization component outputs the current status of the ego vehicle; the perception component outputs the status of surrounding objects. Since the status of objects is directly controlled by the simulator, we can extend the existing simulation interfaces to use the ground truth of objects as idealized substitutes. For prediction components, which are designed to generate predicated future trajectories of surrounding objects, the ground truth is recorded inside the scenario, which can also be available via extending the simulation interface. For the control component, which generates control commands given a planning trajectory, the simulator will use motion models to estimate how the vehicle should move given the control command and then update the vehicle state in simulation. Here, we adapt the Sim-control \josh{Sim-control is capitalized here and in the following sentence it's not} technique from Apollo~\cite{apollo}, which is designed to generate current vehicle states based on planning trajectory \josh{``a planning trajectory'' or ``the planning trajectory''?}. We replace the control component with the sim-control component and directly update the vehicle states in the simulation with sim-control's outputs. 


\textbf{2. Safety-oriented constraint solving.} Extending the simulation bridge interface may not always work for all components. One example is the planning component. The output of the planning component (i.e., planning driving trajectory) cannot extract from simulation, thus we can not directly figure out what is the idealized output of planning. To solve this problem, we follow prior works in planning area~\cite{paden2016survey} and use a constraint-solving problem as the best efforts \josh{``best efforts'' is used awkwardly here. I don't know what you mean.} to find a collision-effort planning trajectory. The constraint-solving problem solved in the idealized substitute of planning is to find a planning trajectory $(W_1, t_1), (W_2, t_2), ... (W_n, t_n)$ (here $W_i$ is a waypoint and $t_i$ is a timestamp) \josh{This sentence is incomplete}
%\josh{Equation \ref{eqn:csp_planning} is oddly specified }
\begin{equation}
\label{eqn:csp_planning}
\begin{aligned}
\text{subj. to} ~ & W_0 = ego\_position \\
& W_n = goal\_position\\
& collision\_free(W_i, t_i) ~ ~ \forall 1\leq i \leq n\\
& D(W_i) ~ \forall 1 \leq i \leq n\\
\end{aligned}
\end{equation}
Here, $collision\_free$ is a function to check the collision with any objects around won't happen at waypoint $W_i$ at time $t_i$ and $D$ is the constraint of vehicle dynamic (e.g., the velocity and acceleration should be within a reasonable range). Compared with the original planning component implementation, the constraint-solving problem is a reduced problem since some non-safety properties of trajectories (e.g., comfort, smoothness) is not considered anymore. We argue that such safety-oriented reduction can reduce possible safety-violation due to consideration of other trajectories properties and should be considered as the best efforts \josh{``best efforts'' is used awkwardly here. I don't know what you mean.}of avoiding safety violations. 
\subsection{Vehicle Dynamic State-based Analysis}
\label{design:state}
To address \textbf{C2}, we propose to cluster the messages based on the vehicle dynamic. The vehicle dynamic is the combination of the vehicle's position, velocity, and acceleration. The reason we adopt a vehicle dynamic is because when two messages are generated under very similar vehicle dynamics, the inputs (i.e., sensor data, localization of ego vehicle) should be similar. The fault should also occur when the inputs are similar. 

For each recorded message, we can collect the vehicle dynamic and then calculate the vehicle dynamic state (we use "state" in the remaining of the paper):
\begin{equation}
    State(p, v, a) = p/p_{unit} || v/v_{unit} || a/a_{unit}
\end{equation}
where $p$, $v$, and $a$ are the position, velocity, and acceleration, respectively, of the ego vehicle and $p_{unit}$, $v_{unit}$, and $a_{unit}$ are pre-defined hyper-parameters. With this definition, we can cluster the messages into different states. 

For example, suppose that we have collected two driving records $T_A$ and $T_B$ under exactly the same safety-violation scenario configuration. In trace $T_A$, a planning message $M1$ is generated when ego vehicle is at position $(3m, 1m)$ and in trace $T_B$, a planning message $M2$ is generated at position $(3.1m, 1.05m)$. The ego vehicle's velocity and acceleration when generating $M1$ and $M2$ are exactly the same. Intuitively, the inputs of the two messages are very similar and if one message is violation-inducing in one trace, the other message is likely to be violation-inducing in the other trace. If we set $p_{uit} =0.2m$, we will have the same states for both messages. After applying state-based cause attribution, even though we can not directly replace the exact messages in the original safety-violation record directly, we are still able to replace messages which likely to induce the same fault and thus further attribute the cause on the message level. 

\subsection{Message-level Cause Attribution Algorithm}
\label{design:localization_algorm}
We present our algorithm of message-level cause attribution in Algorithm.~\ref{alg:cause_localization}. We applied delta debugging~\cite{zeller2002simplifying} into our problem context since we also aim to find minimal changes in the testing setup to flip the testing result. 

The inputs to the algorithm are a sequence of states in the original safety-violation traces. Our algorithm gradually reduces the cause attribution scope by calling $attribute$ function recursively. $attribute$ function takes three arguments: $start$, $end$ represents the boundary of our current cause attribution scope and $step$ is used to decide how we will split the current scope for further recursion. From lines 6 to 9, we will examine two intervals $[start, start~+~step~-~1]$ and $[end~-~step~+~1, end]$. Also, we will check the complement of the aforementioned intervals (line 10 to line 13). If replacing messages in any interval can lead to non-violation testing results, we should reduce our cause attribution scope into that interval. If we can not reduce our scope to any interval, we will reduce the $step$.  

In Fig.~\ref{fig:framework}, we provide a simple example to illustrate our algorithm. We assume that there are 4 states in safety-violation traces. The first test case is generated on line 6. in Algorithm~\ref{alg:cause_localization}. The algorithm first replaces all the messages with idealized component substitutes. However, the safety violation still happens, meaning that the messages in the first two states are not the cause. The next test case is generated on line 8 where messages inside states 3 and 4 are replaced with idealized component substitutes. The testing results show that the safety violation is gone after the replacement, indicating that the cause is inside states 3 and 4. Once reduce the cause to states 3 and 4, we also reduce the step to 1 to gain a more fine-grained cause attribution result. Later, the 3rd test case is generated on line 6. Since the step is already 1, our algorithm will only replace the messages in state 3 with idealized component substitutes. The testing result shows that only the replacement of messages in state 3 can eliminate the safety violation, meaning that we find the minimum states which is the cause. 
\begin{algorithm}
\caption{Message-level cause attribution}\label{alg:cause_localization}
%\hspace*{\algorithmicindent} 
\textbf{Input:}     
A sequence of all states $S1$, $S_2$, ... $S_n$ in original record\\
%\hspace*{\algorithmicindent} \\
\textbf{Output:} 
Two state index indicating the range of faulty messages causing the safety-violation \\
$M_{[a, b]}$ is the set of all messages in states from state $a$ to state $b$.
\begin{algorithmic}[1]
\footnotesize
\Procedure{attribute}{start, end, step}
\If{step = 0}
\State return start, end
\EndIf
\State return {}
\If{rtest($M_{[S_{start}, ~ S_{start ~ + ~ step-1}]}$) = \cmark}

\algorithmiccomment{Reduce the cause to $[start, start ~ +~ step-1]$}
\State return attribute(start, start + step - 1, step/2)
\ElsIf{rtest($M_{[S_{end~-~step~+~1}, ~ S_{end}]}$) = \cmark}

\algorithmiccomment{Reduce the cause to $[end~-~step~+~1, end]$}
\State return attribute(end - step + 1, end, step/2)

\ElsIf{rtest($M_{[S_{start~+~step}, ~ S_{end}]}$) = \cmark}

\algorithmiccomment{Reduce the cause to $[start~+~step, end]$}
\State return attribute(start + step, end, (end - start - step)/2)

\ElsIf{rtest($M_{[S_{start}, ~ S_{end~-~step}]}$) = \cmark}

\algorithmiccomment{Reduce the cause to $[start, end~-~step]$}
\State return attribute(start, end - step, (end - start - step)/2)


\Else 
\State return(start, end, step/2)
\EndIf
\EndProcedure


\State{return attribute(1, n, n/2)}
\end{algorithmic}

\end{algorithm}

==> formulation_prev.tex <==
\section{problem definition}

In this section, we will introduce the problem formulation and assumptions of our proposed cause attribution method. 
\subsection{Application Scenario} 
The main scope of our cause attribution is to understand the cause behind the collision incidents discovered in simulation testing. Additionally, we argue that the proposed techniques can also be applied for cause attribution in closed facility testing and on-road testing via reconstructing the testing scenario in simulation. Waymo claimed that they have reviewed data from crash databases and naturalistic driving studies to
identify other possible collision scenarios and develop tests in simulation~\cite{waymo_safety_report}. Moreover, simulation has been used to reconstruct and analyze real-world collision incidents~\cite{ubercrashreport}. Thus, we believe system failures happen in closed facility testing, on-road testing, and real-world \josh{How is ``real-world'' different from closed facility or on-road? Do you really need to say ``real-world''?} can also be analyzed in simulation environments. 
We focus on collision incidents since they are the most critical and severe system failures of AD systems. These types of incidents endanger human safety and are critical risks after deployment of AD systems~\cite{uber_acquire, ubercrashreport}.

%We assume that the collision is caused by bugs or imperfection in the AD software design and implementation. \josh{Assuming causes come from a particular place is a weird thing to say in an SE paper. This is something we want to determine in these kinds of papers generally, not assume.}
The types of causes this work focuses on include program implementation bugs or imperfection of the machine learning models used for object detection, prediction, and other tasks in AD software. Prior work has demonstrated that the implementation bugs may happen in different modules in AD systems~\cite{garcia2020comprehensive}. Also, imperfect detection results are natural for machine learning models and a few real-world crash cases have demonstrated that such imperfect results can lead to severe collisions~\cite{ubercrashreport, tesla_crash_texas, tesla_crash_truck}.

\subsection{System Requirements}

We assume that the simulation environment can replay the collision scenarios for error attribution purposes. For the simulation testing setup, the testing framework can simply record the testing configuration (i.e., moving trajectories of surrounding objects, map, initial localization of ego vehicle), and it can be used to precisely reproduce the collision scenario for further analysis. For closed facility testing and on-road testing, the testing team can still reconstruct the scenarios by analyzing the collected data via sensors equipped on ego vehicle and sensors installed around the testing facility.

We model each simulation testing execution as a function:
\begin{equation}
collision(S, E)\in \{ True, False\}
\end{equation}
Here $S$ the testing scenario given to the simulator and can be represented as $(map, object\_list, routing)$, where $map$ is the virtual environment created in simulation, $object\_list$ is a list of surrounding objects and corresponding moving trajectories, and $routing$ indicates the routing command given to the AD system. $E$ can be represented as $(perc, pred, plan, cont, loc)$ \josh{Let's use $loc$ instead of $loca$ since the latter means crazy lady in Spanish}, which is a combination of concrete implementation of each core module to control the ego vehicle. The goal of simulation testing is to find a set of collision scenarios where for each element $s_c$ in this set, $collision(s_c, E) = True$. 
\subsection{Error Attribution Goal}
Our design target is to automatically diagnose which module is the root cause of the collision between the AD vehicle and other objects on the road. The result reduces the manual effort needed to debug AD systems and quickly find the correct development and maintenance team to fix this system failure.

However, due to the noisy inputs in AD systems, the errors may happen simultaneously in different modules. For example, inaccurate bounding box detection in the perception module and an imperfect control command can contribute to a collision together. In this case, our goal is to find the minimal set of modules that contain errors leading to the collision.



==> old_background.tex <==
\section{Background and Motivation}
\begin{figure*}[t]
    \centering
    \includegraphics[width=\linewidth]{figure/AD_overview.pdf}
    \caption{\modify{Overview of representative ADS systems and the interactions between its internal components.}}
    \label{fig:ad_framework}
\end{figure*}

\subsection{ADS and Typical ADS Components}

Autonomous Vehicles (AVs), or self-driving cars, are already a reality in our daily life --- over 60 companies are testing such systems on public roads today~\cite{dmv-permit-autox}, and quite a few already in the commercial stage, with notable examples of robo-taxis~\cite{waymo-one, baidu_driverless_robotaxi}, buses~\cite{baidu_bus_service, uk_bus}, trucks~\cite{tusimple-truck, aurora_truck}, and delivery vehicles~\cite{nuro_charge_delivery_service}, not to mention the millions of Autopilot-equipped Tesla cars~\cite{tesla_sold_2_million_cars}.

To achieve safe and correct driving autonomy in complex and dynamic driving environments, the ADS in the AV industry today typically adopt a \textit{multi-component architecture}~\cite{waymo_safety_report, aurora_safety_report, gmcruise_safety_report, apollo, autoware}, where each component is in charge of a relatively self-contained AI functionality and frequently interacts with each other to realize an end-to-end ADS mission, typical via \textit{messages} in a robotic middleware such as ROS~\cite{quigley2009ros}. Fig.~\ref{fig:ad_framework} shows a representative industry ADS architecture with the following core components:

\begin{itemize}[leftmargin=*,nosep]
\item \textbf{Perception} gains an understanding of the environment by processing sensor inputs. Detecting and estimating the states (e.g., position, velocity) of surrounding objects (e.g., pedestrians, vehicles) is the necessary step for an AD vehicle to react to complex driving scenarios. The inputs of perception components are the data collected from sensors equipped by the AD vehicles (e.g., camera, LiDAR). The outputs include the type, position, size (usually in the form of bounding boxes), and velocity of the objects. 

\item \textbf{Prediction} is designed to predict the future trajectories of surrounding objects. It takes the outputs from perception components and generates a list of candidate prediction trajectories to indicate the potential future moving tendency of the object. A Deep Neural Network (DNN) is usually used in both perception and prediction components.

\item \textbf{Localization} is designed to determine the position of the ego vehicle via using sensor data (e.g., IMU, GPS, LiDAR).

\item \textbf{Planning} takes all the environmental information gathered by Perception, Prediction, and Localization and generates a planning trajectory for the ego vehicle. The generated trajectory should obey traffic laws and common driving practices. More importantly, this component is in charge of making decisions to avoid collision with on-road objects. 

\item \textbf{Control} is designed to generate control commands for the vehicle based on planning output.
\end{itemize}

\modify{During the execution, each component will store the subscribed messages, and the main logic of each component will be executed driven by the clock or a certain type of message. Eventually, the output of each execution will be sent to other components as an output message via the APIs provided by the middleware. We can use the following triad to define an execution of a certain component:

\begin{equation}
    e \;:= \;<\, M_{input}, \, m_{output}, \, t>
\end{equation}
where $M_{input}$ is a collection of all the input messages for that program execution, $m_output$ is the output message of the program execution, and $t$ is the timestamp when the output message is published.

During the execution of a driving scenario, each component will continuously collect and transmit messages such that the whole AD vehicle can understand and react to the complicated environment in real time. Thus, the executions of each component will naturally come into a set. We define the execution sets of each component as $E^{perc}$, $E^{pred}, E^{plan}, E^{cont}, E^{loca}$ for perception, prediction, planning, control, and localization component respectively Furthermore, the whole execution of the ADS system could be represented as a matrix:
\begin{equation}
\mathbb{E} = \begin{bmatrix}
e^{perc}_1 & e^{perc}_2 & e^{perc}_3 & ... & e^{perc}_{|E_{prec}|} \\
e^{pred}_1 & e^{pred}_2 & e^{pred}_3 & ... & e^{pred}_{|E_{pred}|} \\
e^{plan}_1 & e^{plan}_2 & e^{plan}_3 & ... & e^{plan}_{|E_{plan}|} \\
e^{cont}_1 & e^{cont}_2 & e^{cont}_3 & ... & e^{cont}_{|E_{cont}|} \\
e^{loca}_1 & e^{loca}_2 & e^{loca}_3 & ... & e^{loca}_{|E_{loca}|} \\

\end{bmatrix}
\end{equation} \alfred{consider using curled brackets?}
where $e_i^X$ means the execution from component $X$ with $ith$ \alfred{$i$-th} smallest timestamp. Each row in this matrix is the execution from the same component sorted with the timestamp. Each component may have a different number of executions even during the same time period, which means the number of elements on each row may vary. For the convenience of presentation, we align the last execution of each component in the matrix representation. 
}



\subsection{Scenario-based Testing for ADS Safety}

Considering that cars are heavy, fast-moving, and operating in public spaces, safety has always been the most important concern for AV developers and policy-makers. To address this, end-to-end system-level safety testing has been one of the most critical steps in the real-world development and deployment of ADS. Road testing is the most natural approach for such safety testing, but due to the large variety of corner-case scenarios and their rarity in naturalist driving, such testing has been widely recognized to be extremely inefficient. For example, it is estimated that an ADS must drive hundreds of millions of miles to validate the safety at the level of human-driven vehicles~\cite{kalra2016driving}, which makes it intractable in practice.

To address this, \textit{scenario-based testing} has been proposed and widely adopted in the AV industry, where the testers can simulate the rare corner-case driving scenarios, typically in a high-fidelity simulator, to test a given ADS with flexibility and scalability. For example, Waymo has reported more than 15 billion miles of such virtual testing of their ADS in their proprietary, high-fidelity simulator~\cite{waymo_safety_report}; Aurora claimed that such a method enables them to perform 2.27 million unprotected left turns in simulation before even attempting one in the real world, which is the key to develop and deploy their ADS safely, quickly, and broadly~\cite{aurora_scale_simulation}. \alfred{draw connections to the problem targeted in this paper}


%Software fault localization is one of the (if not the) most expensive, tedious and time consuming activities in program debugging



%\subsection{AD Software Framework}
%Due to the complexity of the system and cooperation among different development teams and companies, AD software typically applies multi-component architecture, including leading AD companies (e.g., Waymo~\cite{waymo_safety_report}, Aurora~\cite{aurora_safety_report}, GM Cruise~\cite{gmcruise_safety_report}) and popular open-source AD software frameworks (e.g., Baidu Apollo~\cite{apollo}, Autoware~\cite{autoware}). Also, prior works also conducted a systematic analysis of interviews with people who are developing or testing AD software and the results show that all the interviewees are working with multi-component architectures since end-to-end driving models can not handle complicated driving scenarios and often suffer from generalizability issues. 

%In such multi-component architectures, each \textit{component} is a stand-alone program that communicates with other components by sending \textit{messages} (i.e., inputs or outputs of the program) frequently via some middleware (e.g., ROS, cyberRT~\cite{quigley2009ros, apollocyber}). The necessary components of AD systems include: 


%The relationship of different components have been demonstrated in Fig.~\ref{fig_sim_overview}.\todo{Add a polished AD system overview fig}
\begin{comment}
\begin{figure*}[t]
    \centering
    \includegraphics[width=\linewidth]{Fig/simulation_testing_framework.pdf}
    \vspace{-0.22in}
    \caption{Overview of simulation testing on AD system\todo{This is a temp draft}}
    \label{fig_sim_overview}
    \vspace{-0.15in}
\end{figure*}
\end{comment}

\cut{
\subsection{Testing AD Systems}
%\ziwen{I gave up the three types of testing in ~\cite{feng2020testing} (UMhic's works). Instead, I think citing a FSE paper and follow their term might be better.}

Based on the prior survey~\cite{lou2021testing}, there are three commonly used testing methods for AD systems: unit testing, field operational testing, and simulation testing. The developers can manually label and clip driving records from simulation or field operational tests to construct unit tests for control logic and DNN models~\cite{lou2021testing}. However, to verify the safety property of an entire system, we still need to rely on field operational testing or simulation testing. Simulation testing has been widely deployed by AD companies. Even though the environment and vehicle dynamics may be different in the physical world, it is an irreplaceable approach due to its low cost, high efficiency, and also the capability to turn one single physical-world case into thousands of opportunities to practice and improve AD software~\cite{waymo_safety_report}. More background information in this line of research is included in a recent survey~\cite{testing_survey}. Among them, a few recent works~\cite{autofuzz, li2020av} have built heuristic-based algorithms to boost the bug discovery process, and they are able to find safety-violation scenarios for popular open-source multi-component AD frameworks (e.g., Apollo, Autoware~\cite{apollo, autoware}). 

We also want to highlight a few key differences that make AD simulation testing particularly different from traditional software testing: (1) The outputs of AD simulation testing is a scenario configuration, which is the inputs to the simulator instead of inputs to the program under test. (2) The oracle is defined at the system level (e.g., collision), which is a joint effect caused by all components of AD software and simulator. \josh{Please describe why you are highlighting these differences.}



\begin{comment}
Due to the importance of safety in AD systems, testing of AD software has been extensively studied in both academia and industry. Currently, AD testing can be conducted in three approaches: simulation testing, closed facility testing, and on-road testing~\cite{feng2020testing}. Simulation testing has been widely deployed by AD companies. Even though the environment and vehicle dynamic may be different in the real world, it is an irreplaceable approach due to its low cost, high efficiency, and also the capability to turn one single real-world case into thousands of opportunities to practice and improve AD software~\cite{waymo_safety_report}. More background information in this line of research is included in a recent survey~\cite{testing_survey}. \end{comment}
}

%\subsection{Debugging in AD software}



\begin{comment}
Due to the severity of the failures in AD systems, it is highly desirable to have an automated analysis tool that can attribute the error to each component. 
\end{comment}
\begin{comment}
\outline{
Motivation of cause localization in AD software

- Reason 1: reduce the debugging effort, unnecessary to launch hervy-weight simulation

- Reason 2: Further apply other existing software testing/fault localization/fixing technologies

Cause localization in AD software is hard 

- Reason 1: The cause/fault will not happen at the same time as the collision. Since the consequences of fault is propagated among different components in AD systems and physical environment and eventually lead to collision

- Reason 2: Lack of oracles. cite ICST 2020

-- A detection/prediction inaccuracy is common due to the noisy and uncertain of CPS

-- Inaccuracy may not be the cause of collision

Current status of system level debugging
- Cite ICRA 2021, only reducing the environments.
Limitations, can not provide locate the cause and thus can not have the benefits claimed previously

}
\end{comment}

\subsection{Motivation}
\begin{figure}[t]
      \centering
          \includegraphics[width=1.\linewidth]{figure/motivation_example.pdf}  
	\caption{\modify{Illustration of collision between vehicle controlled by the AD software and the pedestrian. (a). shows the moving trajectories of both the vehicle and the pedestrian in the accident. (b)-(e) shows the autonomous vehicle's classification and prediction results of the pedestrian and its corresponding decision. The figures are generated based on the description in NTSB's investigation report~\cite{ntsb_report}.} \josh{Instead of ``Static others object", which is an awkward use of English, the term from the text ``unknown static obstacle" is much better.}\ziwen{Modify the image accordingly.}}
		\label{fig:moti_example}
\end{figure}


We introduce a motivating example to demonstrate how isolating failure-inducing input is different in the AD context compared with general software debugging. This example is a real fatal collision between a vehicle operated by AD software and a pedestrian pushing a bicycle by her side. Being the first pedestrian fatality involving an AD vehicle, this is one of the most high-profile AD collisions in the world. The report by the National Transportation Safety Board (NTSB)~\cite{ntsb_report} explains how it happened. As shown in Figure~\ref{fig:moti_example}.a \alfred{a more common way of subfigure reference is ``Fig. 2 (a)''}, the vehicle had a collision with a pedestrian when she was crossing the road. 5.2 seconds before the collision (Figure~\ref{fig:moti_example}.b), the AD vehicle detected the pedestrian for the first time and mistakenly recognized the pedestrian as a static vehicle. When it was 1.5 seconds before the collision, the pedestrian had 
% come into the current lane of the AD vehicle, 
% it still mistakenly classified the pedestrian as some unknown static obstacle.
entered AD vehicle's lane, and she was again mistakenly classified as some unknown static obstacle.
The AD vehicle generates a planning trajectory to avoid the collision with the static obstacle. However, since it mistakenly thought the object was static, that collision-avoidance planning trajectory could not really avoid the collision once the pedestrian moved closer to the AD vehicle. Finally, when it was 1.2 seconds before the collision, the AD vehicle realized that the collision might happen and claimed an emergency situation. 
% The report claims that alternative classification results will clear the tracking history of the pedestrian, which leads to incorrect prediction.
The report claims that alternative\alfred{alternative or alternating} classification cleared the tracking history of the pedestrian, which led to an incorrect prediction of the pedestrian's trajectory, and ultimately caused the fatal collision.

%Understanding the root cause of this accident is complicated since there is a causality chain coming from the first mistake in the system, propagating through components and time dimensions, and eventually putting the AD vehicle into an emergency situation. On one side, a small error will be used as the input to the next component thus leading to system safety violation iteratively. In this example, it seems that the direct cause of the collision is misprediction of the pedestrian's moving trajectory. However, if we do not loop deep into detailed log and execution information, we cannot figure out the causality relationship between the wrong classification results and the misprediction, thus ignoring the true root cause of the accident. On the other side, the real problem actually occurs much earlier than the collision and the classification result seems quite reasonable at the collision moment since the pedestrian was pushing the bicycle and if the AD vehicle always recognizes the object as the bicycle, it should be able to avoid the moving bicycle. There is an urgent need to build an automated tool to understand the causality relationship between component inputs/outputs along the driving trace to understand the real root cause of the safety violation. 

Understanding the root cause of this accident is far from trivial. Just by looking at the accident description (Figure ~\ref{fig:moti_example}.a), many possibilities exist. The pedestrian was not detected, the pedestrian's tendency towards the AD vehicle was mistakenly ignored, the decision was too aggressive to avoid the collision or even the control command may have contained an error such that the AD vehicle was out of the control of AD software. If our step can go one step further and we are able to see how AD vehicle's internal decision information (Figure ~\ref{fig:moti_example}.b-e), we can clearly exclude some of the assumptions. For example, we can confirm that the pedestrian is detected and the root cause should not be the control command error since the vehicle correctly follows the planning trajectories. However, we still can not confidently conclude the root cause. Even though we know the prediction trajectory is wrong, we can not tell whether this error is an inherent error inside the AD's prediction component or caused by the misclassification results from the perception component. Furthermore, there is also the possibility that the planning component was not ready to handle the pedestrians who 
% goes across the road where he shouldn't. 
are jaywalking.
A natural way to further understand the cause of this accident is to raise some what-if questions: "What if the perception component does not misclassify the pedestrian?" or "What if the prediction component always generates the correct prediction trajectory?". In this paper, we will demonstrate how we understand the root cause of AV accidents by asking and answering the what-if questions. 

Another motivating factor for our work is the automation of the entire process. Given the potentially large volume of data contained in a driving trace \alfred{give number to best show the scale of such ``large volume''}, the need for iterative reduction of the debugging scope through continuous exploration of "what-if" questions becomes essential. This underscores the necessity of an automated approach. 
%\Yuqi{I feel this paragraph is a bit too short to be here, do you prefer to rephrase the last sentence of the previous paragraph as `by asking and automatically answering the what-if questions.'}
The components of ADS are running at a high frequency due to the requirement of quick response in such safety-critical systems. Thousands of messages could have been generated within 10 seconds. \alfred{need evidence; also not sure if this is repetitive to the ``large volume of data'' described above} Let only each message also contain rich information. For example, one single planning message could contain more than one thousand lines of data. \alfred{not sure what you mean by ``lines''} To avoid such heavy manual efforts, an automated framework is necessary for this critical task.

==> result_table.tex <==
\begin{table}[]
\centering
\caption{Evaluation results on benchmark.}
\label{tab:result}
\begin{tabular}{lllll}
\hline
           & \begin{tabular}[c]{@{}l@{}}Component-level\\ accuracy\end{tabular} & \begin{tabular}[c]{@{}l@{}}Sound\\ -ness\end{tabular} & \begin{tabular}[c]{@{}l@{}}Complete\\ -ness\end{tabular} & \begin{tabular}[c]{@{}l@{}}Reduction\\ rate\end{tabular} \\
\hline
Perception   & 100\%                                                           & 0.97                                                  & 0.71                                                     & 0.94\%                                                   \\
\hline
Prediction   & 100\%                                                           & 0.94                                                  & 0.63                                                     & 1.07\%                                                   \\
\hline
Planning     & 100\%                                                           & 0.93                                                  & 0.74                                                     & 0.87\%                                                   \\
\hline
Control      & 100\%                                                           & 0.92                                                  & 0.51                                                     & 6.79\%                                                   \\
\hline
Localization & 100\%                                                           & 0.87                                                  & 0.57                                                     & 4.29\%        \\
\hline
\end{tabular}
\end{table}
